ERUP-YOLO: Enhancing Object Detection Robustness for Adverse Weather Condition by Unified Image-Adaptive Processing

We propose an image-adaptive object detection method for adverse weather conditions such as fog and low-light. Our framework employs differentiable preprocessing filters to perform image enhancement suitable for later-stage object detections. Our framework introduces two differentiable filters: a B\'ezier curve-based pixel-wise (BPW) filter and a kernel-based local (KBL) filter. These filters unify the functions of classical image processing filters and improve performance of object detection. We also propose a domain-agnostic data augmentation strategy using the BPW filter. Our method does not require data-specific customization of the filter combinations, parameter ranges, and data augmentation. We evaluate our proposed approach, called Enhanced Robustness by Unified Image Processing (ERUP)-YOLO, by applying it to the YOLOv3 detector. Experiments on adverse weather datasets demonstrate that our proposed filters match or exceed the expressiveness of conventional methods and our ERUP-YOLO achieved superior performance in a wide range of adverse weather conditions, including fog and low-light conditions.

==> tabs/ablation_foggy.tex <==
\begin{table}[t]
    \centering
    \tiny
    \caption{Results}
    \label{tb:res_fog}
    \begin{tabular}{lccc}
    \\
    &{\scriptsize V\_n\_ts}&{\scriptsize V\_f\_ts}&{\scriptsize RTTS}\\
    &{\scriptsize (mAP)}&{\scriptsize (mAP)}&{\scriptsize (mAP)}\\
    \\
    \hline
    \\
    {\scriptsize BPW}&{\footnotesize 76.67}&{\footnotesize 72.35}&{\footnotesize 48.22}\\
    \\
    {\scriptsize KL}&{\footnotesize {\bf 77.35}}&{\footnotesize {\bf 74.68}}&{\footnotesize 49.89}\\
    \\
    {\scriptsize BPW+KL}&{\footnotesize \underline{77.04}}&{\footnotesize \underline{72.71}}&{\footnotesize {\bf 49.95}}\\
    \\    
    \end{tabular}
\end{table}

==> tabs/ablation_lowlight.tex <==
\begin{table}[t]
    \centering
    \tiny
    \caption{Results}
    \label{tb:res_fog}
    \begin{tabular}{lccc}
    \\
    &{\scriptsize V\_n\_ts}&{\scriptsize V\_d\_ts}&{\scriptsize ExDark}\\
    &{\scriptsize (mAP)}&{\scriptsize (mAP)}&{\scriptsize (mAP)}\\
    \\
    \hline
    \\
    {\scriptsize BPW}&{\footnotesize 66.85}&{\footnotesize 57.85}&{\footnotesize  47.97}\\
    \\
    {\scriptsize KL}&{\footnotesize \underline{67.85}}&{\footnotesize {\bf 59.08}}&{\footnotesize {\bf 48.93}}\\
    \\
    {\scriptsize BPW+KL}&{\footnotesize {\bf 68.38}}&{\footnotesize \underline{58.95}}&{\footnotesize \underline{48.76}}\\
    \\    
    \end{tabular}
\end{table}
